Aspects of Polar-Coded Modulation

We consider the joint design of polar coding and higher-order modulation schemes for ever increased spectral efficiency. The close connection between the polar code construction and the multi-level coding approach is described in detail. Relations between different modulation schemes such as bit-interleaved coded modulation (BICM) and multi-level coding (MLC) in case of polar-coded modulation as well as the influence of the applied labeling rule and the selection of frozen channels are demonstrated.

==> ch_conclusion.tex <==


\section{Summary and Outlook}%\vspace*{2mm}

In this paper we have given a structured approach to polar-coded modulation.
We have discussed similarities and equivalences on a conceptual level.
These insights have been utilized to optimize polar-coded BICM and MLC.

Several points remain open for optimization of polar-coded modulation.
A starting point for this optimization is the selection of frozen channels in the polar code construction matched to the higher-order constellation, as motivated in this paper.
To this end, we believe that the similarity of the transformation of Gray into SP labeling with the polar code construction can be exploited benefically.
Finally, the incorporation of fading channels appears to be an important task for future work.



==> ch_intro.tex <==

%
\section{Introduction}
\label{sec:intro}
%


The need for bandwidth-efficient coded modulation for modern communication systems is evident.
This raises the question of the optimal combination of modulation and channel coding.
To some extent this problem has been settled through the use of bit-interleaved coded modulation (BICM)~\cite{BICM:Caire:BICM}.
In BICM coding and modulation are designed almost independently: a channel code optimized for the binary input AWGN channel is connected via a mapper and (possibly) an interleaver with a higher-order modulation scheme.

Compared to the optimal joint design of coding and modulation following the so-called multi-level coding (MLC) principle~\cite{IT:WachsmannFischerHuber:Multilevelcodes}, BICM induces only a small loss in capacity.
However, in particular for realistic finite-length codes, employing codes optimized for the binary-input AWGN channel instead of those optimized for the higher-order system at hand leads to significant performance degradation.
This is well understood, e.g., for the application of convolutional codes, where channel codes optimized for trellis-coded modulation outperform conventional BICM approaches~\cite{IT:Ungerboeck:TCM}.
For other coding schemes, especially those mainly developed after Caire's fundamental paper on BICM in 1998~\cite{BICM:Caire:BICM}, such as turbo codes and low-density parity check codes, this problem has hardly been addressed.

The unique structure of polar codes~\cite{Polar:Arikan} offers promising starting points for joint optimization of coding and modulation (so-called \emph{polar-coded modulation}).
This makes polar codes -- if correctly designed -- very attractive for coded modulation schemes, apart from  their well-known benefits  (in particular,  the low-complexity encoding and decoding).

The aim of this paper is to show first results of and motivate a thorough approach to polar-coded modulation.
To this end, we discuss and contrast the application of polar codes in MLC and BICM. 
We point out benefits and similarities from an information-theoretic conceptual point of view.
Building on the relation of Gray and natural labeling, recently shown in~\cite{BICM:Alvarado:Equivalence},  we proof the equivalence of polar-coded BICM and MLC for $4$-QAM under the constraint of equal structural delay.
We underline the importance of a polar code construction optimized for the applied modulation scheme, i.e., in particular the optimized selection of so-called frozen channels.
The observations are supported by means of numerical results.
Based on these insights, we motivate points for further optimization of polar-coded modulation.

For sake of clarity and in order to facilitate our approach, we restrict ourselves to the additive white Gaussian noise (AWGN) channel.
The transfer of insights gained for this setup to different channel models, especially incorporating fading scenarios, is an interesting task for future research.

This paper is organized as follows:
After a brief review of the main building blocks in Sec.~\ref{sec:model},
we discuss the application of polar codes in multi-level and bit-interleaved coded modulation in Sec.~\ref{sec:MLC} and \ref{sec:BICM}, respectively.
Our main findings are summarized in Sec.~\ref{sec:results}.
The paper concludes with an outlook.

